Towards automated kernel selection in machine learning systems: A SYCL case study

Automated tuning of compute kernels is a popular area of research, mainly focused on finding optimal kernel parameters for a problem with fixed input sizes. This approach is good for deploying machine learning models, where the network topology is constant, but machine learning research often involves changing network topologies and hyperparameters. Traditional kernel auto-tuning has limited impact in this case; a more general selection of kernels is required for libraries to accelerate machine learning research. In this paper we present initial results using machine learning to select kernels in a case study deploying high performance SYCL kernels in libraries that target a range of heterogeneous devices from desktop GPUs to embedded accelerators. The techniques investigated apply more generally and could similarly be integrated with other heterogeneous programming systems. By combining auto-tuning and machine learning these kernel selection processes can be deployed with little developer effort to achieve high performance on new hardware.

==> Makefile <==

PACKAGE = auto-kernel-sel-2020
NAME = auto-kernel-sel
SECTIONS = \
					 introduction.tex \
					 matmul.tex \
					 pruning.tex \
					 classification.tex \
					 conclusions.tex \
					 future_work.tex \

IMAGES = \
				 images/max_config_counts.png \
				 images/pca_variance.png \
				 images/data_distribution.png \
				 images/error_vs_classes.png \
				 images/classifiers.png \
				 images/results_vgg.png \
				 images/results_mobilenet.png \
				 images/results_resnet.png \
				 images/seen_results_vgg.png \
				 images/seen_results_mobilenet.png \
				 images/seen_results_resnet.png \

all: ${NAME}.pdf

%.pdf: %.tex ${SECTIONS} ${IMAGES} ${TABLES} bibliography.bib
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	  do pdflatex $<; done

clean_pictures:
	$(RM) ${IMAGES}

images/max_config_counts.png: scripts/plot_max_counts.py
	python3 scripts/plot_max_counts.py

images/pca_variance.png: scripts/plot_pca_variance.py
	python3 scripts/plot_pca_variance.py

images/error_vs_classes.png: scripts/plot_error_classes.py data/model_classes.csv
	python3 scripts/plot_error_classes.py

images/classifiers.png: scripts/plot_classifiers.py data/classifiers_dtree.csv
	python3 scripts/plot_classifiers.py

images/data_distribution.png: scripts/plot_all_data.py
	python3 scripts/plot_all_data.py

images/results_vgg.png: scripts/plot_model_perf.py data/results.csv
	python3 scripts/plot_model_perf.py data/results.csv images/results

images/results_mobilenet.png: scripts/plot_model_perf.py data/results.csv
	python3 scripts/plot_model_perf.py data/results.csv images/results

images/results_resnet.png: scripts/plot_model_perf.py data/results.csv
	python3 scripts/plot_model_perf.py data/results.csv images/results

images/seen_results_vgg.png: scripts/plot_model_perf.py data/seen_results.csv
	python3 scripts/plot_model_perf.py data/seen_results.csv images/seen_results

images/seen_results_mobilenet.png: scripts/plot_model_perf.py data/seen_results.csv
	python3 scripts/plot_model_perf.py data/seen_results.csv images/seen_results

images/seen_results_resnet.png: scripts/plot_model_perf.py data/seen_results.csv
	python3 scripts/plot_model_perf.py data/seen_results.csv images/seen_results

clean:
	$(RM) *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	*.tar.gz

archive: all clean
	COPYFILE_DISABLE=1 \
		tar -C .. -acf ../$(PACKAGE).tar.gz \
		--exclude '*~' \
		--exclude '*.tar.gz' \
		--exclude '*.tgz' \
		--exclude '*.zip' \
		--exclude '.git*' \
		--exclude '$(PACKAGE)/data' \
		--exclude '$(PACKAGE)/scripts' \
		--exclude '*.pdf' \
		$(PACKAGE)
	mv ../$(PACKAGE).tar.gz .

